STT-CBS: A Conflict-Based Search Algorithm for Multi-Agent Path Finding with Stochastic Travel Times

We present an algorithm for finding optimal paths for multiple stochastic agents in a graph to reach their destinations with a user-specified maximum pairwise collision probability. Our algorithm, called STT-CBS, uses Conflict-Based Search (CBS) with a stochastic travel time (STT) model for the agents. We model robot travel time along each edge of the graph by independent gamma-distributed random variables, and propose probabilistic collision identification and constraint creation methods to robustly handle travel time uncertainty. We show that under reasonable assumptions our algorithm is optimal in terms of expected sum of travel times, while ensuring an upper bound on each pairwise conflict probability. Simulations and hardware experiments show that STT-CBS is able to significantly decrease conflict probability over CBS, while remaining within the same complexity class.

==> 6_Bibliography.tex <==
\begin{thebibliography}{6}
%

\bibitem{cbs}
Sharon, G., Stern, R., Felner, A., Sturtevant, N.R.:
Conflict-based search for optimal multi-agent pathfinding.
Artificial Intelligence,
Vol. 219, No.1, pp. 40-66 
(2015)

\bibitem {cbsta}
Hönig, W., Kiesel, S., Tinka, A., Durham, J.W., Ayanian, N.: 
Conflict-Based Search with Optimal Task Assignment. 
In Proceedings of the International Conference on Autonomous Agents and Multi-Agent Systems (AAMAS).
International Foundation for Autonomous Agents and Multiagent Systems, 757–765 
(2018)

\bibitem {cbsheuristics}
Felner, A., Li, J., Boyarski, E., Ma, H., Cohen, L., Kumar, T. S., Koenig, S.:
Adding heuristics to conflict-based search for multi-agent path finding. 
International Conference on Automated Planning and Scheduling
(2018)

\bibitem{disjointcbs}
Li, J., Harabor, D., Stuckey, P. J., Ma, H., Koenig, S.:
Disjoint splitting for multi-agent path finding with conflict-based search. 
International Conference on Automated Planning and Scheduling, Vol. 29, No. 1, pp. 279-283
(2019)

\bibitem{smtcbs}
Surynek, P.:
Unifying search-based and compilation-based approaches to multi-agent path finding through satisfiability modulo theories. 
In Annual Symposium on Combinatorial Search
(2019)

\bibitem {Korn}
Kornhauser, D., Miller, G., Spirakis., P.: Coordinating pebble motion on graphs, the diameter of permutation groups, and applications. 
In Annual Symposium on Foundations of Computer Science, pp. 241-250
(1984)

\bibitem {cap}
{\v C}{\'a}p, M.:
Centralized and Decentralized Algorithms for Multi-Robot Trajectory Coordination [Doctoral thesis]. Czech Technical University in Prague, 147p.
(2017)

\bibitem{flow}
Yu, J., LaValle, S. M.: Optimal multirobot path planning on graphs: Complete algorithms and effective heuristics. 
IEEE Transactions on Robotics, 32(5), pp. 1163-1177
(2016)

\bibitem{bayen}
Krichene, W., Reilly, J., Amin, S., Bayen, A.:
On the characterization and computation of Nash equilibria on parallel networks with horizontal queues.
IEEE Conference on Decision and Control (CDC)
(2012)

\bibitem{robustcbs}
Atzmon, D., Stern, R., Felner, A., Wagner, G., Barták, R., Zhou, N. F.: Robust multi-agent path finding. 
In Annual Symposium on Combinatorial Search
(2018)

\bibitem{probustcbs}
Atzmon, D., Stern, R., Felner, A., Sturtevant, N. R., Koenig, S.: 
Probabilistic robust multi-agent path finding.
International Conference on Automated Planning and Scheduling, pp. 29-37
(2020)

\bibitem{delayprobabilities}
Ma, H., Kumar, T.K. S., and Koenig, S.: Multi-agent path finding with delay probabilities. 
AAAI Conference on Artificial Intelligence, pp. 3605-3612
(2017)


\bibitem{YuNPHard}
Yu, J.: 
Intractability of optimal multirobot path planning on planar graphs. 
IEEE Robotics and Automation Letters, 1(1), 33-40
(2015)

\bibitem{cbm}
Ma, H., Koenig, S.: 
Optimal target assignment and path finding for teams of agents. arXiv preprint:1612.05693.
(2016)

\bibitem{pushnrotate}
De Wilde, B., Ter Mors, A.W., Witteveen, C.: 
Push and rotate: a complete multi-agent pathfinding algorithm. Journal of Artificial Intelligence Research, 51, pp. 443-492
(2014)

\bibitem{odid}
Standley, T.S., Korf, R.: 
Complete Algorithms for Cooperative Pathﬁnding Problems. International Joint Conference on Artificial Intelligence
(2011)

\bibitem{warehousemanagement}
Wurman, P. R., D'Andrea, R., Mountz, M.: 
Coordinating hundreds of cooperative, autonomous vehicles in warehouses. AI Magazine, 29(1), pp. 9-9
(2008)

\bibitem{warehousedesignoptimization}
Ashayeri, J., Gelders, L. F.:
Warehouse design optimization. European Journal of Operational Research, 21(3), pp. 285-294
(1985)
 
\bibitem{uav}
Ho, F., Geraldes, R., Goncalves, A., Cavazza, M., Prendinger, H.:
Simulating shared airspace for service UAVs with conflict resolution. 
International Conference on Autonomous Agents and MultiAgent Systems, pp. 2192-2194
(2018)

\bibitem{routingstochastictt}
Samaranayake, S., Blandin, S., Bayen, A.: 
A tractable class of algorithms for reliable routing in stochastic networks. 
Transportation Research Part C: Emerging Technologies, 20(1), pp. 199-217
(2012)

\bibitem{cocktailapproach}
Lumelsky, V. J., Harinarayan, K. R.: 
Decentralized motion planning for multiple mobile robots: The cocktail party model. 
Autonomous Robots, 4(1), pp. 121-135.
(1997)

\bibitem{astar}
Hart, P. E., Nilsson, N. J., Raphael, B.:
A formal basis for the heuristic determination of minimum cost paths. 
IEEE Transactions on Systems Science and Cybernetics, 4(2), pp. 100-107
(1968)

\bibitem{nphard}
Yu, J., LaValle, S. M.: Structure and intractability of optimal multi-robot path planning on graphs. 
AAAI Conference on Artificial Intelligence
(2013)


\bibitem{cbslargeagents}
Li, J., Surynek, P., Felner, A., Ma, H., Kumar, T. S., Koenig, S.:
Multi-agent path finding for large agents. In Proceedings of the AAAI Conference on Artificial Intelligence, Vol. 33, pp. 7627-7634
(2019)

\bibitem{umstar}
Wagner, G., Choset, H.:
Path planning for multiple agents under uncertainty. International Conference on Automated Planning and Scheduling
(2017)

\bibitem{mstar}
Wagner, G., Choset, H.:
M*: A complete multirobot path planning algorithm with performance bounds. In IEEE/RSJ international conference on intelligent robots and systems, pp. 3260-3267
(2011)

\bibitem{ouijabots}
Wang, Z., Yang, G., Su, X., Schwager, M.:
Ouijabots: Omnidirectional robots for cooperative object transport with rotation control using no communication. 
In Distributed Autonomous Robotic Systems, pp. 117-13, Springer.
(2018)

\bibitem{rvo2}
Van Den Berg, J., Guy, S. J., Lin, M., Manocha, D.: Reciprocal n-body collision avoidance. 
Springer Tracts in Advanced Robotics, Vol. 70, pp. 3-19
(2011)

\end{thebibliography}

==> Alg_2_MostLikelyConflict.tex <==

\begin{algorithm}
 \caption{Most Likely Conflict}
 \begin{algorithmic}
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand\algorithmicthen{}
 \renewcommand\algorithmicdo{}

 \STATE \textit{Fill the graph with occupancy information}:
  \FOR {each edge traversed by agents in $S$}
  \STATE Add occupancy information to the graph at nodes and edges: agent $R$, expected arrival time $t$, shape factor $n$
  \ENDFOR
 \STATE $P_{c_{max}} = \epsilon$
 \STATE MostLikelyConflict = $\emptyset$
  \FOR {each occupied vertex and edge in the graph}
  \FOR {each of their pairwise, possibly conflicting occupants}
  \IF{considered element is an edge}
  \STATE Search for adjacent edges traversed by both agents
  \STATE Combine these edges
  \ENDIF
  \STATE Calculate $P_{conflict}$ using (\ref{nodeprobability}) or (\ref{edgeprobability})
  \IF {$P_{conflict} \geq P_{c_{max}}$}
  \STATE MostLikelyConflict = Conflict(concerned agents, planned times of arrival)
  \STATE $P_{c_{max}}$ = $P_{conflict}$
  \ENDIF
  \ENDFOR
  \ENDFOR
 \STATE \textbf{return} MostLikelyConflict
 \end{algorithmic} 
 \label{mlcalg}
 \end{algorithm}

==> Alg_3_Dichotomy.tex <==

\begin{algorithm}
 \caption{ \textcolor{blue}{Constraint From Conflict}}
 \begin{algorithmic}
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand\algorithmicthen{}
 \renewcommand\algorithmicdo{}
 

 \STATE $t_{A1} \gets$ time at which agent $a_i$ planned to arrive at the node or edge
 \STATE $n_1 \gets$ delay parameter for agent $a_i$
  \STATE $t_{A2} \gets$ time at which the other agent planned to arrive at the concerned element
 \STATE $n_2 \gets$ delay distribution parameter for the other agent
 \STATE $P_{conflict} \gets 1.0$
 \STATE $d_1 \gets 0$
 \STATE $d_2 \gets$ Arbitrarily large number
 \WHILE{$P_{conflict} > \epsilon$ \textbf{or} $ \mid P_{conflict} - \epsilon \mid \geq $ tolerance}
 \STATE $ d \gets \frac{1}{2}(d_1+d_2)$
 \STATE $P_{conflict} = P_{cm}(t_{A1}+d - t_{A2},n_1,n_2,t_2,n_m,\lambda)$ or $P_{conflict} = P_{ce}(t_{A1}+d - t_{A2},n_1,n_2,t_2,\lambda,t_e)$
  \IF {$P_{conflict} \geq \epsilon$}
  \STATE $d_1 \gets d$ 
  \ELSE {}
  \STATE $d_2 \gets d$ 
  \ENDIF
 \ENDWHILE
 \STATE \textbf{return} Constraint(R1, element, $d$)
 \end{algorithmic} 
 \label{dichalg}
 \end{algorithm}
